Bounded Satisfiability for PCTL

While model checking PCTL for Markov chains is decidable in polynomial-time, the decidability of PCTL satisfiability, as well as its finite model property, are long standing open problems. While general satisfiability is an intriguing challenge from a purely theoretical point of view, we argue that general solutions would not be of interest to practitioners: such solutions could be too big to be implementable or even infinite. Inspired by bounded synthesis techniques, we turn to the more applied problem of seeking models of a bounded size: we restrict our search to implementable -- and therefore reasonably simple -- models. We propose a procedure to decide whether or not a given PCTL formula has an implementable model by reducing it to an SMT problem. We have implemented our techniques and found that they can be applied to the practical problem of sanity checking -- a procedure that allows a system designer to check whether their formula has an unexpectedly small model.

==> discussion.tex <==
\section{Conclusion}
\label{sec:discussion}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "cav"
%%% End: 

In this paper, we have introduced the \emph{bounded satisfiability} problem,
which is a simplification of the satisfiability problem for PCTL, that restricts
consideration to models that can be implemented. As was expected, 
bounded satisfiability is NP-complete in the minimal output. To offset this
negative result, we provided a reduction from bounded satisfiability to an SMT
problem, because in practice SMT solvers can often answer large queries.

%Our motivation was to provide means to find simple model---for our formal measure of simplicity: the simplest model---of a PCTL formula was twofold:
%we wanted to enable a system engineer to detect loopholes in formal specifications by providing her with a comprehensible model of the given specification,
%and we wanted to provide a system designer with a simple model to support her during the implementation process.


Our experimental results allow for two interpretations. Our first set of
experimental results shows that the difficulty of finding a solution to the
system of SMT constraints depends strongly on the size of the minimal model.
Hence, we consider it unlikely that these techniques will be able to construct
the large systems that would be useful in practice. On the other hand, our
second set of benchmarks showed that the running time of the SMT solver does not
depend strongly on the size of the PCTL formula. Indeed, we were able to
construct systems that satisfy formulas with hundreds of temporal operators. It
would seem that, while our techniques are not able to construct models that are
large enough be useful in practice, they are able to handle the large
specifications that may appear in this setting. This motivates the idea of
sanity checking, where a system designer wishes to ensure that there are no
errors in a specification that could lead to a small satisfying model. Our
results indicate that our techniques are capable of providing a sanity checking
procedure.

%The speed does not seem to depend primarily on the size of the constraint system, but on the size of the simple model we allow for.
%On the one hand, we always received fast answers for small bounds on the model size, even though we scaled up the constraint systems to ... .
%On the other hand, Yices seems to be very sensitive to the chosen bound.
%This may be because the resulting Markov chain can, at least potentially, grow in measures like tree width \cite{} in the size of the resulting model, and it may just be because the heuristics are not optimised towards this problem class.
%Bounded satisfiability checking might therefore form an interesting class of
%problems for SMT competitions to understand them better, and cooperations
%between researchers interested in SAT/SMT solving and researchers interested in
%the satisfiability and synthesis problems for systems with temporal
%specifications seem to be interesting future work.



==> introduction.tex <==
\section{Introduction}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "cav"
%%% End: 


PCTL \cite{HJ94} is a popular logic for the specification of
probabilistic systems. The model checking problem for PCTL formulas
over Markov chains has been widely studied: it is known to be solvable
in polynomial time%~\cite{HJ94}
, and mature tools, such as PRISM~\cite{DBLP:conf/cav/KwiatkowskaNP11}
and MRMC~\cite{DBLP:journals/pe/KatoenZHHJ11}, have been developed. By
contrast, satisfiability procedures for PCTL have received much less
attention. Recently, it has been shown that the satisfiability problem
for the qualitative fragment of PCTL is
EXPTIME-complete~\cite{BFKK-lics08}. However, the satisfiability
problem for PCTL itself is not even known to be decidable.

%The idea of this paper was born when we took a step back and considered the question, why we would be interested in the satisfiability of a formula.
%On the face of it, the answer is simple: if one has a specification, one is interested in the question of whether or not is has a model, simply because there cannot be an implementation otherwise.
%The crux of this observation is, that we are really interested in the question of whether or not there is an implementation.


%The situation for PCTL satisfiability checking has many similarities.
%We do not even know a general decision procedure, but the problem of whether or not there is a model and whether or not there is a finite model are EXPTIME hard even for the qualitative fragment---and the answer to these questions may be different \cite{}:
%even for the qualitative fragment, some formulas require infinite models such that $0$ is a limit point of the transition probabilities.
%Both of these side constraints obviously exclude implementability.

In this paper, we take a step back, and ask the following question: even if we
could find an algorithm for the satisfiability of PCTL, would it be useful to a
practitioner? We believe that it would not. Even in the qualitative fragment of
PCTL, there are already formulas for which %there is no finite state model, but
%for which there is an infinite state model.
there are only infinite state models. Moreover, the problem of
deciding, for this fragment of PCTL, whether there is a finite model
is EXPTIME-hard~\cite{BFKK-lics08}. Obviously, the situation is at
least as bad for the full PCTL logic.

When practitioners use satisfiability procedures, it is
likely that they are interested in whether their formula has an
\emph{implementable} model. A constructive satisfiability procedure may return
an infinite state model, or a model with bizarre transition probabilities that
may be difficult to implement in practice. Neither of these two situations seems
to be desirable. Hence, our goal is to solve the following problem.

\[\mbox{``Does a PCTL specification $\phi$ have an implementable model?''}\]

Our results are inspired by the work on bounded synthesis for LTL
specifications~\cite{Schewe+Finkbeiner/07/Bounded,Finkbeiner+Schewe/07/smt,Ehlers/10/SymbolicBoundedSynthesis,DBLP:conf/stacs/KupfermanLVY11,ehl11tacas},
where the question of whether there is a small reactive system for an LTL
formula is considered. Building on this, we define the \emph{bounded
satisfiability} problem for PCTL formulas, where the goal is to find a
\emph{simple} model of a PCTL formula. In our setting, a model is simple if it
has a small number of states, and if it uses only rational transition
probabilities that can be easily simulated by, for example, coin tossing. We
believe that having a simple model is a prerequisite for having an implementable
model. Certainly, infinite models, and models whose probabilities cannot be
simulated by coin tossing would not seem to be useful in practice.


%For two reasons, we believe that the simpler an implementation is, the more useful it will be, leading to the \emph{bounded satisfiability} problem that can be phrased as

%Simple refers to additional constraints on its structure, e.g., limiting the number of states and allowing only rational transition probabilities that are easy to simulate, for example, by coin tossing.
%These reasons are the \emph{construction of simple models} and performing a \emph{sanity check of the specification}.


%\paragraph{\bf Simple Models}
%While the quest for simple formalisation errors is inspired by bounded model checking, the construction of simple models is inspired by bounded synthesis \cite{Schewe+Finkbeiner/07/Bounded}.
%Bounded synthesis is the problem of finding a small reactive system that satisfies Church's solvability problem.
%Synthesis for temporal specifications is hard \cite{Pnueli+Rosner/89/Synthesis,Kupferman+Vardi/99/Church}, even undecidable in a distributed setting \cite{Pnueli+Rosner/90/Distributed,Finkbeiner+Schewe/05/Distributed}.


%We therefore argue that, from a practical point of view, only finite models are of interest, because only they can be implemented.
%But even finiteness is an insufficient constraint.
%Ultimately, a model needs to be implemented, and the number of states it can have therefore has practical constraints.
%We therefore argue in favour of seeking small models up front.

\paragraph*{\bf Results} In this paper, we introduce the concept of a simple
model, and the bounded satisfiability problem. This is the problem of finding,
for a given PCTL formula $\phi$ and bound~$b$, a simple model of~$\phi$ with at
most~$b$ states. We provide a reduction from bounded satisfiability to SMT.
While PCTL satisfiability is not known to be decidable, our results
show that the bounded satisfiability problem can be decided. We also provide
complexity results for the bounded satisfiability problem. We show that it is
NP-complete in the size of the minimal model. Furthermore, we show that
approximating the size of the minimal model is NP-hard.

%We have therefore introduced the \emph{bounded satisfiability problem}, where we restrict the joint size of the model and intermediate states needed by a random-number generator that can only toss coins to be no greater than a given threshold.


%We have implemented an academic tool based on the reduction of bounded satisfiability to SMT, using Yices \cite{DBLP:conf/cav/MouraDS07} as a solver, and showed the applicability of our techniques for both motivating cases on a case study.

We have constructed a simple implementation of our reduction from
bounded satisfiability to SMT, and we have solved the resulting
constraint systems using the Yices SMT
solver~\cite{DBLP:conf/cav/MouraDS07}. We tested this implementation
on an academic case study, and our results show that the bounded
satisfiability problem can indeed be solved when the number of states
required is small.

\paragraph*{\bf Practical Applications} While our simple implementation does
show that small models can be found by our techniques, the size of these models
is clearly well below what would be required for constructing systems in an
industrial setting. On the other hand, we argue that a bounded synthesis
procedure for even a small number of states is useful for the purpose of
\emph{sanity checking.}

In model checking, we attempt to verify that a potentially buggy system
satisfies a specification. However, in recent years it has become increasingly
clear that the specification itself may also contain
bugs. See, for example, the work on vacuity
checking~\cite{Beer97efficientdetection,Purandare:2002:VCC:647771.734418,DBLP:journals/sttt/KupfermanV03,AFFGPTV03,DBLP:conf/tap/BallK08}. It can also
be remarkably difficult to detect these errors, since a model checking procedure
will simply output ``yes'' in the case where a buggy system satisfies the buggy
specification.

We propose that bounded satisfiability has a role to play in helping system
designers find bugs in their specifications. Consider, for instance, a
complicated specification of a network protocol that allows, among many other
things, the network to go down and subsequently be recovered. A buggy
specification may allow a model that goes down immediately after service has
been restored, which would allow the model to circumvent most of the
specification. This model will have far fewer states than a model that
implements a correctly functioning network. In this case, while a correct system
may be too large to build with our techniques, it is quite possible that the
broken system could be built.
 
Hence, we propose that bounded satisfiability should be used as a sanity check,
in order to test that a formula does not have an error that can be exploited by
a small model. Suppose that a system designer has a large system that is known
to satisfy some complicated specification. If the bounded satisfiability
procedure produces a small model for the specification, then there is a problem
that can be resolved in one of two ways. Firstly, it may be the case that the
small model does precisely what the designer wants, and in this case the
overly-complex large system can be replaced by the small one. The more likely
outcome is that the small model does not do what the designer intended. In this
case, the designer now has a small, understandable counter-example, which can
be used to help correct the specification.

Our experimental results show that our bounded satisfiability procedure is
particularly suitable for sanity checking. While our implementation does not
seem to scale well with the number of states in the model, it does scales well
with size of the input formula. This indicates that sanity checking may indeed
be possible for the type formulas that are used in practice.

%When performing a sanity check for a specification, we want to identify errors in the formalisation of requirements.
%Consider, for example, a specification of a network protocol that consists of a list of requirements that the network shall satisfy when it is operational, including lower bounds on the likelihood that a system stays operational, as well as the likelihood that it returns to an operational state if it is down.

%It easily happens that one slips in formalising such requirements, introducing, say, a loop-hole that allow the network to frequently go down, thus avoiding to satisfy all `real' requirements while complying with its formal specification.
%Constructing a \emph{simple} model would unearth such specification errors by constructing formally correct systems with obviously undesirable behaviour.

%Avoiding such formalisation errors is an important prerequisite for a formal analysis of the resulting system to be meaningful.
%Naturally, bounded satisfiability checking is not a perfect way to avoid such errors.
%In fact, no perfect way can exist, simply because it is impossible to formalise them.
%It is rather inspired by bounded model checking techniques \cite{Biere+others/03/Bounded,Copty+others/2001/Benefits}, where we only aim at finding simple bugs.

%Finding such bugs, however, cannot be automated, because it requires the analysis of a synthesised model by a system engineer.
%It does, however, imply---slightly fuzzy---constraints on the model presented to her:
%for two reasons, such models should be small.
%First, a big model may not exploit such a loophole, and second, only simple models are accessible to a system analyst.

%For our example with a network protocol, a normal synthesis procedure could, in principle, produce a large model that complies with both the formal specification and the true requirements.
%In such a case, this model would not be helpful in identifying the slip in the formalisation of the requirements.
%But even if the loophole is exploited in an automatically constructed model with millions of states, this slip is very unlikely to be caught.

%As opposed to that, tiny models of complex specifications are usually forced to exploit such slips.
%(Though a suitable model with a handful of states would be a great side result.)
%At the same time, tiny models are open to human analysis, allowing for the identification of specification errors.

%Similar to bounded model checking \cite{Biere+others/03/Bounded,Copty+others/2001/Benefits} or analysis techniques using bounded context switches \cite{DBLP:conf/pldi/MusuvathiQ07,DBLP:journals/fac/HolzmannF11}, this technique cannot be expected to find all bugs, but it will lead to an increase quality of the specification.
%Moreover, and key to the implementability of such approaches, it does not put a high strain on the system analyst.
%For her, the construction of a small model as an alarm the sanity check would raise.
%But the sanity check would raise at most one false alarm, and this would provide the system analyst with a valuable concise model.



%\paragraph{\bf Related Work}
%(As you'll easily see, not what should be here, only space holders)
%
%Bounded Synthesis \cite{Schewe+Finkbeiner/07/Bounded,DBLP:conf/stacs/KupfermanLVY11} has much better implementations than the crap Bernd and I produced at the time \cite{Finkbeiner+Schewe/07/smt}, in particular the  the BDD-based 
%\emph{Unbeast}~\cite{Ehlers/10/SymbolicBoundedSynthesis,ehl11tacas} and the antichain-based tool \emph{Acacia}~\cite{DBLP:conf/cav/FiliotJR09}.
%
%Vacuity: \cite{}
%
%Bounded model checking: \cite{Biere+others/03/Bounded,Copty+others/2001/Benefits}


%\paragraph{\bf Organisation of the Paper}
%After introducing the ... in the preliminaries, we give our problem statement in Section \ref{sec:setting}.
%We describe a reduction from bounded satisfiability to SMT in Section
%\ref{sec:implementation}, followed by a discussion of complexity of our bounded
%satisfiability in the following section.
%Finally, we describe our implementation and present experimental results in Section \ref{sec:implementation}.

